Upper and lower bounds for dynamic data structures on strings

We consider a range of simply stated dynamic data structure problems on strings. An update changes one symbol in the input and a query asks us to compute some function of the pattern of length $m$ and a substring of a longer text. We give both conditional and unconditional lower bounds for variants of exact matching with wildcards, inner product, and Hamming distance computation via a sequence of reductions. As an example, we show that there does not exist an $O(m^{1/2-\varepsilon})$ time algorithm for a large range of these problems unless the online Boolean matrix-vector multiplication conjecture is false. We also provide nearly matching upper bounds for most of the problems we consider.

==> 3sum_hardness.tex <==
\newcommand{\SUM}{\textsc{3SUM}\xspace}
\newcommand{\oSD}{\textsc{oSD}\xspace}

In this section we show lower bounds for \DEM, \DIP, and \DHD conditional on the hardness of the \SUM problem. In this problem we are given a set $S \subset \{-n^3, \dots, n^3\}$ of size $n$ and must decide if there is a triple of distinct $x, y, z \in S$ with $x + y = z$. The modern \SUM conjecture is as follows:

\begin{conjecture}[\SUM Conjecture~\cite{Patrascu:2010:polylower}]\label{conj:3sum}
In the word RAM model with words of $O(\log n)$ bits, for any constant $\eps > 0$ there is no $O(n^{2-\eps})$-time algorithm for the \SUM problem.
\end{conjecture}

As a preliminary step, we introduce the offline Set Disjointness (\oSD) problem. In the \oSD problem we are given a set $C$ of elements, two families $A$ and $B$ of subsets of $C$, and $q$ pairs of subsets $(A_i, B_j) \in A \times B$, and we must determining for each of the $q$ pairs of sets whether they are disjoint or not.

\begin{theorem}[Theorem 1.4 by Kopelowitz et al.\@~\cite{KPP:2016}]\label{thm:Seth}
Let $f(n)$ be such that \SUM requires expected time $\Omega(\frac{n^2}{f(n)})$. For any constant $0 < \gamma < 1$ let $\mathbb{A}$ be an algorithm for \oSD where $|C| = \Theta(n^{2-2\gamma})$, $|A|=|B|= \Theta(n \log n)$, each set in $A \cup B$ has at most $O(n^{1-\gamma})$  elements from $C$, and $q = \Theta(n^{1+\gamma} \log n)$. Then $\mathbb{A}$ requires $\Omega(\frac{n^2}{f(n)})$ time.
\end{theorem}

\begin{theorem}
Assuming the \SUM conjecture, there does not exist an algorithm running in $O(n^{1/4-\eps})$ time for the maximum of query and update time for \DEM, \DIP, and \DHD, for any constant $\eps > 0$. The same lower bound holds even when updates are permitted only in the pattern or only in the text.
\end{theorem}
\begin{proof}
We first give a reduction from \oSD to \DEM. We generate the text $T$ of length $|B| \cdot |C|$ as follows. For each set $B_j \in B$ we create a binary string of length $|C|$ by setting its $i$th bit to $1$ if $i \in B_j$ and $0$ otherwise. The text $T$ is the concatenation of such $|B|$ strings. We initialise the pattern of length $|B| \cdot |C| / 2$ to be all wildcards. 

We group the $q$ queries by which set $A_j \in A$ is a part of the query. For each set $A_j$ we answer the corresponding queries as follows. First we perform $O(n^{1-\gamma})$ updates to the first $|C|$ letters of $P$ so that $P[i] = 0$ if $i \in A_j$, for the remaining $P[i] = \; ?$. To answer the set disjointness query $(A_j, B_k)$ we align the start of the pattern encoding $A_j$ with the start of the encoding of $B_k$ in the text and do an exact match query. If it is not an exact match then there is an $i$ where $P[i]=0$ that is matched to a one, which means element $i$ is both in $A_j$ and $B_k$, i.e. they intersect. Similarly, if it is an exact match then $A_j$ and $B_k$ do not intersect. 

Overall it takes $O(n^{3-2\gamma}\lg n)$ time to create the text and we use $O(t_q \cdot q + t_u \cdot |A| n^{1-\gamma}) = O(t_q \cdot n^{1+\gamma} + t_u \cdot n^{2- \gamma}\lg n)$ to perform the updates and queries, where $t_q$ is the query time and $t_u$ is the update time. For any constant $\eps > 0$, setting $\gamma =\frac{1}{2} + \eps$ we obtain that $T$ can be constructed in $O(n^{2-2\varepsilon}\lg n)$ time. From Conjecture~\ref{conj:3sum} and Theorem~\ref{thm:Seth} it then follows that $O(t_q \cdot n^{\frac{3}{2}+\eps}\log n + t_u \cdot n^{\frac{3}{2}-\eps} \lg n) = n^{2-o(1)}$. Thus $t_q = \Omega(n^{\frac{1}{2} - \eps})$ or $t_u = \Omega(n^{\frac{1}{2} + \eps})$ for a text of size $n^{2-2\eps}\log n$. The lower bound follows. 

Note that in the proof above we do not update the text, so the bound holds for the general model and for the model when updates are permitted only in the pattern. For the text-only updates, we need to swap the pattern and the text. Namely, we generate the pattern $P$ of length $|B| \cdot |C|$ as follows. For each set $B_j \in B$ we create a binary string of length $|C|$ by setting its $i$th bit to $1$ if $i \in B_j$ and $0$ otherwise. The pattern is the concatenation of the $|B|$ strings. The text has length $2 |B| \cdot |C|$, and all its letters are equal to wildcards except for the letters in positions $|B| \cdot |C| - |C| + 1, \dots, |B| \cdot |C|$. As before, we group the $q$ queries by which set $A_j \in A$ is a part of the query. For each set $A_j$ we answer the corresponding queries as follows. First we perform $O(n^{1-\gamma})$ updates to the letters in positions $|B| \cdot |C| - |C| + 1, \dots, |B| \cdot |C|$ of $P$ so that $P[i] = 0$ if $i \in A_j$, for the remaining $P[i] = \; ?$. To answer the set disjointness query $(A_j, B_k)$, we align the start of the encodings of $A_j$ and $B_k$ and do an exact match query. The bound follows.

The lower bound for \DIP follows by reducing \DEM to \DIP. The lower bound for \DHD follows from reduction from \DIP. 
\end{proof}
